PAR: Personal Activity Radius Camera View for Contextual Sensing

Contextual sensing using wearable cameras has seen a variety of different camera angles proposed to capture a wide gamut of different visual scenes. In this paper, we propose a new camera view that aims to capture the same visual information as many of the camera positions and orientations combined from a single camera view point. The camera, mounted on the corner of a glasses frame is pointing downwards towards the floor, a field-of-view we named Personal Activity Radius (PAR). The PAR field-of-view captures the visual information around a wearer's personal bubble, including items they interact with, their body motion, their surrounding environment, etc. In our evaluation, we tested the PAR view's interpretability by human labelers in two different activity tracking scenarios: food related behaviors and exercise tracking. Human labelers achieved an overall high level of precision in identifying body motions in exercise tracking of 91% precision and eating/drinking motions at 96% precision. Item interaction identification reached a precision of 86% precision for labeling grocery categories. We show a high level on the device setup and contextual views we were able to capture with the device. We see that the camera wide angle captures different activities such as driving, shopping, gym exercises, walking and eating and can observe the specific interaction item of the user as well as the immediate contextual surrounding.

==> 7.Results.tex <==
\section{Results}
\subsection{Data Set}

\begin{figure}[t]
  \centering
 \includegraphics[width=0.89\linewidth]{fig/examples_misclassif.jpeg}
  \caption{Examples of potential edge cases for confusion of labeler. We can see instances of objects (two pizzas, pepper, curry, chips) and exercise activities (leg lifts and mountain climbers) from left to right. Those examples might be hard to classify due to the informational gap created by occlusion and missing high resolution.}
  \label{fig:ex_miscl}
\end{figure}

\subsection{Human Labeling Evaluation}
In total, 47 different human labelers performed 1275 classification procedures and made a total of 10536 predictions. We can see that labelers are able to classify specific items, however, different item categories and items within those were hard to distinguish and determine by the workers. Namely packaged items and seasoning and sauces were hard to distinguish by the human intelligence force. The exercise category task was performed successfully, but once again a classification of grocery shopping items yields problems within potentially ambiguous food items. A couple of examples of human intelligence confusion is shown in Figure \ref{fig:conf_ex}. 
In the subsequent sections, we evaluate the different performance of labelers according to our defined algorithm to predict (sub) scenarios and classifications. This evaluation gives insights into the interpret-ability of the observed data and subsequently evaluates the ability to label this data by labelers. We show an overview of the performances of all experiments and the subsequent classifications of important properties seen in our Personal Activity Radius Data set. Figure \ref{fig:overview_acc} shows, that we achieved high accuracies in pose, scenario, food analysis, exercise category and repetitions as well as shopping activities and item count. Classification of exercise activities and shopping categories as well as shopping item classification lead to some confusion of the labelers. All evaluations will be analysed in detail in the following sections.

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{fig/accuracy.jpeg}
  \caption{Overview of the human intelligence evaluation accuracies for the sub categories pose, scenario, exercise, food and shopping analysis.}
  \Description{}
  \label{fig:overview_acc}
\end{figure}

\subsubsection{Scenario Analysis}
The ability to classify a video based on a scenario analysis can be summarized to clear results. We observe that humans achieve an accuracy of  98\% when classifying the different food, shopping or exercise scenarios.
In Figure \ref{fig:scen_conf} we can see that the misclassification of the scenario analysis is low. People seemed to infer the scenario by the given context very precisely. We can see in Figure \ref{tab:scen_conf} that all of the scenarios get similar almost perfect precision, recall and F1-Scores of up to 100 \%. The confusion matrix can be in Figure \ref{fig:scen_conf} and visualizes the almost perfect classification.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.7\linewidth]{fig/scen_prf.png}
  \caption{Confusion matrix and precision, recall, f1-scores for experiments for contextual situation analysis. White boxes indicate zero values.}
  \Description{}
  \label{fig:scen_conf}
\end{figure}

We can conclude by these results that labelers are able to identify the different scenarios we captured with our contextual sensor, namely they are able to distinguish shopping, food and exercise scenarios. The perfect precision indicates that if we desire to capture data with our device and give it to labelers, we will get almost perfect results for potential machine learning applications. The only mis-classification with the `none` label indicated that it would be possible to subsequently filter the labels by this `class` and re-check which labels are actually needed. However, we do not need to fear that the label is mixed up with one of the other scenarios. The amount of instances for this evaluation as well as simple setup for labelers might have contributed to this clear and almost perfect result.


\subsubsection{Activity Analysis}

Activity analysis as a result of out human intelligence algorithm can be evaluated three fold. Since we performed three main exercises, we evaluate three different groups of activities for food, shopping and exercise activities.
Our results in form of a confusion matrix for the activity analysis task can be seen in Figure \ref{fig:act_food_conf}, \ref{fig:act_shop_conf} and \ref{fig:act_exer_conf} for the respective three clusters of activities. For the analysis on the activity level, we observed an accuracy of 94\% for food activities such as taking a bite a sip or touching the face during food intake. We can see that  the precision and recall of the bite and sip activities is almost perfect between 96 and 100\%. We see some confusion between activities involving touching the face. This might be due to the fact that some of our samples included touching the user`s face even with the food item in the user`s hand. We specifically wanted to know how far accurate prediction is possible even in edge cases. 

\begin{figure}[t]
  \centering
  \begin{subfigure}{.49\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{fig/activity_food_prf.png}
  \caption{Food Activity}
  \label{fig:act_food_conf}
\end{subfigure}%
\begin{subfigure}{.51\textwidth}
\centering
  \includegraphics[width=0.9\linewidth]{fig/activity_shop_prf.png}
  \caption{Shopping Activity}
  \label{fig:act_shop_conf}
\end{subfigure}
\caption{Confusion matrices and precision, recall, f1-score for activity analysis, clustered by activity types. White boxes indicate zero values.}
\Description{}
  \label{fig:corr}
\end{figure}

\begin{figure}[t]
  \centering
 \includegraphics[width=0.85\linewidth]{fig/activity_prf.png}
  \caption{Confusion matrices and precision, recall, f1-score for exercise activity analysis. White boxes indicate zero values.}
  \Description{}
  \label{fig:act_exer_conf}
\end{figure}

We observe an accuracy of 91\% for shopping activities such as adding or removing an item from a user`s possession or interacting visually or physically with an item. We can see that there is some confusion between visual inspection and that labelers chose to not classify the given instance as a visual inspection. This might be due to the fact that visual interaction in itself does not have a clear trigger. Physical interaction is defined by the user touching the item, but our contextual sensor does not provide any data on where the user is actually looking at. This is an informational gap which would probably need a further setup to close. We thus explore a limit of our contextual sensor.

The gym exercise activity recognition performed worse than the other activity classifications. This cluster performed with an accuracy of 70\%. We can  see that there is confusion in the exercise activities. Those were hard to classify without previous knowledge of the potentially unique gym poses which may or may not be known by the general labeler without prior information on this task (e.g. mountain climbers or leg lifts). We can also see that there was confusions between activities with similar motions, such as pull ups and weight lifting machines for arm musculature. We can see some images of exercises which lead to confusion in Figure \ref{fig:ex_miscl}.

We can see for all activity cluster, that most confusion happened with the none categorization. This hints again on the fact that the interpret-ability and reliability of the provided classifications is high, but might need to be post-checked to fill in gaps which could not be interpreted by untrained labelers for very specific tasks.

\subsubsection{Clustering Activities and Items into Categories}
The analysis of clustering exercise activities into categories yields to an accuracy of  85\%. We can see that few confusions happened between the categories which again lead to a high precision for most categories. Machines have a lower precision with 86\% which might be due to the fact that we did not cover many different machines in our sample (we covered three weight lifting machine exercises but for example six body weight exercises.)

\begin{figure}[b]
  \centering
  \begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{fig/cat_exerc_prf.png}
  \caption{Exercise Category}
  \label{fig:cat_ex_conf}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
\centering
  \includegraphics[width=\linewidth]{fig/cat_shopp_prf.png}
  \caption{Shopping Item Category}
  \label{fig:cat_shop_conf}
\end{subfigure}
\caption{Confusion matrices and precision, recall, f1-score for category analysis. White boxes indicate zero values.}
\Description{}
  \label{fig:cat_shop_conf_all}
\end{figure}


The analysis of clustering grocery items into category performed with an accuracy of 71\%. We can see that there is some confusion within the packaged food section as well as for seasoning an junk food. This might be due to the variety of product within these categories, which are not defined by a clear and unique shape. For example a banana will always have the same elongated shape, but cookies can have many forms and packages which might hide the actual content of the package. Even names and descriptions could be hidden by motion artifacts or missing resolution of the camera setup, which makes it harder to infer the content. We can see the confusion matrices in Figure \ref{fig:cat_shop_conf_all}.

We can nevertheless conclude that it is possible for labelers to infer exercise activity categories and grocery item clusters from our provided data. Similarly to the above cases we might need some post check up to label not identifiable instances. What is different for this evaluation though is that there is information missing on packaged products, which hinders a perfectly reliable classification.


\subsubsection{Item Classification}
As we have seen in item category performance, we observe that the actual item identification classification had similar recall issues than the item category classification. This implies that it was hard for labelers to distinguish packaged items such as chips as well as seasoning and sauce items such as salt and pepper. The food items were predicted correctly with an accuracy of 69\%. The confusion matrix for this classification can be found in Figure \ref{fig:obj_shop_prf} in the appendix.
We can observe that the precision of the classification is high across the board, but the recall is low for certain items. Since most of this mis-classification occurred in the `none` class, this indicates that if using labelers within an open guided classification algorithm might need a post classification by the experiment designer to fill in missing items that could not be identified by labelers. We can see some images of objects which lead to confusion (salt, curry, chips) in Figure \ref{fig:ex_miscl}.


\subsubsection{Item in Hand Counting}
In the grocery shopping task, for tasks where the subject was asked to pick up an item, they were also instructed to grab from 1 to 5 of the same item. The amount of items a user held in their hand was counted correctly with an accuracy of 94\% and the correlation can be seen in Figure \ref{fig:corrob}. The standard deviation from the true value for this evaluation is 0.56 items. We can see that labelers tend to under predict the amount of items chosen by the user. This might be due to the fact that items could be hidden below other items. Figure \ref{fig:ex_miscl} shows an instance of the user holding two pizzas, however only one is visible because they are stacked.

\subsubsection{Exercise Repetition Counting}
A subset of exercises are repetition based, with the subjects performing 10 repetitions per exercise. The videos were segmented by the data collector and a sequence was shown to the Turker to include a random number of repetitions. The labelers correctly counted the number of repetitions in 89\% of the cases, with a correlation coefficient of R = TODO[X], RMSE of TODO:[X], and Standard Deviation of 1.8 repetitions. The correlation of the repetition counting is shown in \ref{fig:objsh}. 

\begin{figure}[b]
  \centering
  \begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{fig/correlation_items.png}
  \caption{Correlation matrix for the item count repetition analysis.}
  \label{fig:objsh}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
\centering
  \includegraphics[width=\linewidth]{fig/correlation_reps.png}
  \caption{Correlation matrix for the exercise repetition analysis.}
  \label{fig:corrob}
\end{subfigure}
\caption{Correlation matrices of the exercise and item count repetition analysis. Color intensity indicates correlation intensity, so a darker grey/black indicates that more labeler predicted this number, whereas a lighter grey indicated that only few labeler predicted this value.}
\Description{}
  \label{fig:corr}
\end{figure}


\subsubsection{Food Intake Content Recognition}
We evaluated the food intake recognition for the food and liquid intake based on the item contents provided by the human classifier and checked these evaluations with the given labels. Since we analysed a given whole meal, this problem allowed multi label classification. We evaluated this multi label classification using a one hot encoding and a one vs rest evaluation technique for each ingredient and checked whether the labeler correctly predicted the existence of the content in the meal. We analysed the evaluation of least one of the items was classified correctly reached an accuracy of 94\%. All items contents were classified correctly with an accuracy of 82\%. We subsequently analysed the precision, recall and f1-score for the specific meal contents. We can see that the precision is high across the board, but the recall of food ingredients is low. All precision, recall and f-1 scores are shown in Figure \ref{table:food_prf}.

\begin{table}
\begin{tabular}{l|rrr}
\toprule
{} &  Precision &  Recall &  F1-Score \\
\midrule
Fruit        &        100\% &      57\% &        72\% \\
Meat         &         75\% &      30\% &        43\% \\
Vegetables   &         80\% &      35\% &        48\% \\
\midrule
Salty Snacks &         85\% &      77\% &        81\% \\
Sweets       &        100\% &      19\% &        32\% \\
Fast Food    &         81\% &      52\% &        64\% \\
\midrule
Water  &         90\% &     100\% &        94\% \\
Coffee &         90\% &     100\% &        94\% \\
Soda   &         70\% &      94\% &        80\% \\
\bottomrule
\end{tabular}
\caption{Precision, recall and f1-score of the nutritional content drinks and food experiment.}
\label{table:food_prf}
\end{table}


\subsubsection{Pose Estimation}
The poses, observed across all experiments, are classified accurately in 91\% of the cases, whereas the more common poses are classified correctly more often than poses like reaching up or bending down. Additionally, we observed more instance of standing and sitting than more edge case like poses like reaching up and bending down which leads to an unbalanced data set. We can see that standing, lying and sitting is classified with 96 to 100\% precision and high recall. Reaching up, bending down and crouching however lead to more confusion.  The confusion matrix of the pose estimation is shown in Figure \ref{fig:pose_conf}. 

\begin{figure}[h]
  \centering
  \includegraphics[width=0.8\linewidth]{fig/pose_prf.png}
  \caption{Confusion matrix and precision, recall, f1-score for pose estimation  for contextual analysis. White boxes indicate zero values.}
  \Description{}
  \label{fig:pose_conf}
\end{figure}

\subsection{Machine Classification Evaluation}
Our transfer learned model was able to predict scenarios with 98\% accuracy and thus matched the accuracy observed by labelers.
\begin{figure}[h]
  \centering
  \includegraphics[width=0.8\linewidth]{fig/scen_prf_ML.png} 
  \caption{Confusion matrix and precision, recall, f1-score for automated machine learned scenario classification for contextual analysis. White boxes indicate zero values.}
  \Description{}
  \label{fig:pose_conf}
\end{figure}

==> Backup.DataClassification.tex <==
\section{Dataset and Labeling}
\subsection{Dataset}
Our dataset consists of 321 labeled videos, including 87 minutes and 109,620 frames of data. This data is labeled with the performed pose, scenario, primary interaction item, item category, activity category, activity and activity repetition. We successfully collected all the previously defines properties of Personal Activity Radius Data that we set to observe. We collected data 'between the scenes' so the labeled videos are a subset of the whole data set we collected. The total data set is a super set of the labeled data set and contains 190 minutes or 239,400 frames of (partly unlabeled) data of our specified activities as well as null activities. These unlabeled instances were not included in our analysis but were nevertheless made available for public further processing in our github repository. Some example of the collected data from different exercises and in different environments can be found in Figure \ref{fig:examples}. We can see activities according to Figure \ref{fig:tree} such as driving a car, walking stairs, picking up items, for example apples and orange juice at a grocery store (left four columns). We can see sit ups and leg lift exercises performed as well as a user sipping on a coke and eating a burger and fries (right four columns). The images are displayed in an order from top to bottom to indicate the temporal movement of the activities, behaviors and interactions of the user, which are subsequently to be classified to the respective pose, item, activity and food label. Figure \ref{fig:examples} shows only a frames of the many we collected. Our data set includes a variety of different lighting conditions, behaviors and motion patterns performed by different people as well as variations of location. The full temporal video representation can be seen in the attached video or in our github repository.

\subsection{Human Labeling}
The focus of our work is to evaluate the potential for using the PAR field of view for vision based activity recognition. Instead of focusing on implementing the computational implementation for specific applications, we believe that a more effective investigation is around the human labelability of this visual data. This is for two reasons. First, the major advancement of computer vision based activity tracking and scene understanding has come from the fact that such a data can be labeled using crowd-sourcing as people can transfer human knowledge to a dataset that was not collected by themselves. In this way, our evaluation focuses on demonstrating the label-ability of videos captured using this view point such that it would be possible to curate labeled datasets for future applications without the need for rigorous in the moment labeling. Data collection can happen simply by wearing the camera day to day and labeled through crowd work. A second reason for looking at human label-ability is for a common use case of deploying wearable cameras for annotating activities in a study or journaling scenarios. As suggested by Bedri et al. in Fitbyte, the purpose of their glasses mounted camera is not for automatic classification and identification of food item, but rather as a means for the user to reflect and self journal. By demonstrating that the scene, object, pose, and activity is identifiable by even someone who did not perform the task is a strong indication that the images captured can be utilized in these scenarios too.

To test the label-ability of our dataset, we used the Amazon Mechanical Turk platform to ask labelers a set of questions that starts at the top level scenario and move down more and more granular.The questions are organized in the flow as shown in Algorithm 1 with a graphical decision tree shown in Figure \ref{fig:overview_acc}. The information shown to the labeler is only a video segment showing a single context. This single context has been labeled at the time of data collection by the data collector, the person's pose, the scenario they are in, and the activity they are performing. This label acts as the dataset's oracle. The pose of the person includes: standing, sitting, laying down, crouching, bending over, and reaching their arm overhead. The scenario includes the three application scenarios we tested: grocery shopping, exercising at the gym, and eating food. Finally the activity classification is dependent on the scenario. 

For grocery shopping, we asked the labeler four questions. First is what is the INTERACTION. The kinds of interaction in the dataset includes inspecting an item visually without touching it (visual), physically inspecting an item (physical), taking the item into possession (add), and removing the item from possession (remove). Next, we ask the labeler what is the CATEGORY of the item. Category refers to the broader class that an item falls under. The full list of categories are listed in Figure \ref{fig:tree}. Based on the category selected, the labeler is then asked to choose the specific ITEM under the category. For example, under the category produce, the labeler is shown apples, bananas, peaches, strawberries, blueberries, lettuce, potatoes, onions, bell peppers, and broccoli. The list of items comes from the full list of items that were collected in our dataset as identified by the oracle. Finally, if the INTERACTION chosen is taking an item into possession, the labeler is also asked to count the number of items. 

For gym exercises, we asked the labeler three questions. First is what is the exercise EQUIPMENT being used, which includes body weight, free weights, weight machines, and cardio machines. Next, based on the equpiment chosen, a more detailed EXERCISE list is presented. For example, if the labeler chose body weight, the list presented includes plank, leg lift, jumping jacks, pull ups, push ups, mountain climber, and sit ups. Finally, if the exercise chosen is one that has REPETITIONS, such as push ups or bicep curls, the labeler is asked to count the number of repetitions. 

For food eating, we asked the labeler two questions. First is b

The framing of the question is around if the labeler sees if a particular context exist. So in this way, if a labeler believes that none of the contexts listed is in the video, then they can label it as NONE. NONE can be selected for any question. So if someone thinks they see produce and selects produce for the category, but do not think any of the items in the list is the produce they see, they can selected NONE. In this way, we are able to analyze from a view point of precision and recall of the labels for all levels of our labeling tree. 

We decided for a top down approach due to the advantage that when a broader structure is identified, we can make a more fine grained contextual analysis and establish important connections between the steps of the top down approach.
Researchers found out that humans typically try to use simple classification strategies and only move to more complex structures if needed \citep{rogers2010humans, johansen2002there}. This has the advantage of computational efficiency \citep{jarecki2018naive} as well as allowing contextual analysis to be a multi-step process. 


%starting from a scenario to an object granularity, as shown in Figure \ref{fig:tree}. For example, we first ask if the scenario happened in one of the three big categories (shopping, exercise, food), and then ask which activity was performed and lastly item or activity category following by item content or repetition count (if any) was seen in the scene. The following algorithm describe in \ref{algo} describes the linear sequence of questions that were asked to the human intelligence workers. Every data point is meant to be classified by three different human intelligence workers. We did not provide any exemplary data sample for the human intelligence workers to orientate on. Thus, the human labelers did not have prior information on the task. We also included tasks of with different amount of labels to choose from. Thus we can see how well the human labelers perform with different question setups. Human intelligence worker always had the possibility to choose not to answer the question or to that none of the provided labels fits to the video content. An example of one classification procedure for one instance is shown in Figure \ref{fig:example_algo} and shows the run through the  algorithm from a broad to fine scale for one instance of the shopping scenario, namely someone interacting physically with one pint of ice cream. 
\IncMargin{1em}
\begin{algorithm}[b]
\SetKwData{Category}{category}\SetKwData{ItemNumber}{itemNumber}\SetKwData{ActivityType}{activityType}\SetKwData{Item}{item}\SetKwData{Pose}{pose}\SetKwData{Repetitions}{repetitions}\SetKwData{ItemContent}{itemContent}\SetKwData{Scenario}{scenario}
\SetKwFunction{AskForScenario}{askForScenario()}
\SetKwFunction{AskForAT}{askForActivityTypeAndCategory(c.\Category)}
\SetKwFunction{AskForIE}{askForItem(exercise)}
\SetKwFunction{AskForIF}{askForItem(foodDiary)}
\SetKwFunction{AskForIS}{askForItem(shopping)}
\SetKwFunction{AskForP}{askForPose(c.\Scenario)}
\SetKwFunction{AskForR}{askForRepetitions(exercise)}
\SetKwFunction{AskForIC}{askForItemContent(foodDiary)}
\SetKwFunction{AskForIN}{askForItemNumber(shopping)}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{A video $v$ of size $width\times height \times time$}
\Output{A classified context $c$ including category, activity type and category, pose, repetitions, interaction item, number of items and content}
\BlankLine
Context c\;
c.\Pose\leftarrow\AskForP;\;\\
c.\Scenario\leftarrow\AskForScenario;\;\\
c.\ActivityType\leftarrow\AskForAT;\;\\
\BlankLine
\Switch{c.\Scenario}{
\uCase{exercise}{
c.\Item\leftarrow\AskForIE;\;\\
c.\Repetitions\leftarrow\AskForR;\;\\
}
\uCase{shopping}{
c.\Item\leftarrow\AskForIS;\;\\
c.\ItemNumber\leftarrow\AskForIN;\;\\
}
\uCase{foodDiary}{
c.\ItemContent\leftarrow\AskForIC;\;\\
}
\Other{
\Return{c}\;
}
}
\Return{c}\;
\caption{Human Intelligence Classification Algorithm }
\label{algo}
\end{algorithm}\DecMargin{1em}


==> Backup.ExperimentalSetup.tex <==
\section{Experimental Setup}

To collect the data to evaluate the PAR video perspective, we recruited 6 participants (3 female, 3 male) to participate in 3 different scenarios: exercise, shopping, and eating. For data collection and labeling, we setup a Raspberry Pi connected to the glasses as a web server. This setup allows the wearer of the PAR glasses untethered from the data collector, with the data collector being able to view and label the recording on a mobile phone while observing the subject. The web server is based the implementation of Melchior et al \citep{mel2013rpi}. We supplemented the existing software with a custom labeling interface. The frame rate was set to 21 fps at 1500x1125 resolution. 

\subsection{Shopping Activity}
In the shopping activity scenario, the experiment is designed to observe a subject during grocery shopping. We defined the grocery item list capturing the following categories: produce, liquids, animal products, frozen food, packaged food, seasoning, sauces, and junk food. The shopping list was designed to represent a variety of items from a western diet. The subject can interact with the item in 4 ways: taking the item into possession, putting the item back, inspecting the item, and standing in-front of the item without touching it. Finally, we also randomize the pose of the person when they interact with the item from reaching up, bending down, and crouching. 

The interface randomly assigns the item, method of interaction, pose, and the number of items to get between 1 to 5. The data collector informs the subject of the next assignment, tags the start of the activity, announces to the subject to start, and tags the end of the activity when the subject completes the assignment. To minimize mislabeling, the subject is first instructed to get close to the item to be interacted with before the label is tagged. To diversify the duration of interaction, subjects were in addition cued to either interact with the item quickly (<1 second) or for a longer duration (inspect the item for a self-determined 2-5 seconds). Each participant visited one grocery store, with one of the participants visiting two grocery stores, providing data for seven different grocery stores. In total, we collected TODO[stats about the dataset]

 \begin{figure}[b]
  \centering
  \includegraphics[width=\linewidth]{fig/tree.jpeg}
  \caption{Based on out literature review, we found several everyday activities suitable and interesting to connect contextual traits with. This tree visualises the properties observed within our 3 experiments exercise, food and shopping analysis.}
  \Description{}
  \label{fig:tree}
\end{figure}

\subsection{Exercise Activity}
In the exercise activity scenario, the experiment is designed to observe a subject doing a variety of exercises in an indoor gym environment. The activities included different categories including body weight, dumb bells, weight machines, and cardio machines. Figure 5b shows the full list of exercises under each category. Activities that are repetition based (e.g. push-ups, arm curls) are performed for ten repetitions. Activities on cardio machines are performed for one minute. Exercises were performed in a randomized sequence. The exercise assignment is announced to the subject in the same way as the shopping activity. TODO[stats about data collected. Number of different exercises, total repetitions, total duration]

\subsection{Eating Activity}
In the eating activity scenario, the experiment is designed to observe a subject during a eating situation where they freely consume food item of their choice (i.e. ordered food, self-prepared food, or snack). We observed each person within a 5-minute eating interval and annotate each bite and sip. The general macronutrient content for food items were annotated. The labels include carbohydrates, fruits, vegetables, meat, fish, eggs, dairy. For liquids, the labels include water, milk, coffee, tea, soda, alcohol. We further annotate if the food item is fast food, snacks, or sweets. We additionally labeled the user's pose during eating. To add additional complexity to the data, we also collected instances of the subjects just bringing their hand to their face without eating or drinking. TODO[Stats about the data collected. Different food items. Different drink items. Number of bites and sips]


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix


==> _5.Evaluation_OLD.tex <==
\section{Evaluation}
 In this paper, we evaluate the system by looking at a number of prototypical activity and context recognition and tracking scenarios. In each scenario, we designed a set of usecases to capture how the visual data looks in the PAR view. The evaluation focuses on examining the label-ability of the visual data by crowd-sourced human labelers. The label-ability of the visual data is extremely important as further development of automated systems that would look towards using PAR as the source of visual data would require labeling of the scene based on their application. If the visual information captuerd by PAR is too difficult to interpret by human labelers, it would mean that videos would need to be labeled at the time of capture to distill the data collector's interpretation of the scene, losing one of the biggest strength of vision-based analysis. The different scenarios help to reveal aspects around the PAR view in regards to tasks commonly desired for visual computing such as object identification, body motion and posture analysis, and the visibility and interpretability of the surrounding. We suspect that end-applications would dictate the type of algorithm ultimately employed, but the label-ability of different components of the scene that we examine here provides a generalizable understanding of how our solution can provide machine learnable visual data.
 

 %We identified three different scenarios that are common in the wearable activity tracking community: shopping, exercise tracking, and eating. Each of these scenario we chose a set of typical metrics of interest. Each of these scenarios were also chosen to both feature the strengths of PAR and also to examine its limitations. For shopping, identifying the category and food item a person interacts with and being able to determine how the person interacts with an item requires the item to both be in-frame, have enough detail, and interpretable in the top-down view point.  Exercise tracking requires the visual information to capture different movements of the body, the equipment/objects being used, and the repetition of the exercise movement. Eating tracking is a diverse task that involves tracking the how you eat, such as bite tracking and context of eating (e.g whether you are eating while commuting, eating while socializing, eating in solitude), and the content of what you are eating. In each of these scenarios, we conducted a user study where subjects engaged in a scenario specific activity and collected videos captured from our prototype PAR glasses. Videos are labeled by crowdsourced human labelers using Amazon Mechanical Turk for the different activities. In the following sections, we breakdown the evaluation based on each scenario. Finally, as we envisioned, we believe that the end usecase and development pattern around the use of PAR would be for application designers to focus on developing virtual sensors around the PAR view. As such, we also evaluate, in the frame of these three scenarios, distinguishing which scenario virtual sensor would best fit the current view.
 
%=========================Scenario 1 ===========================%
\subsection{Scenario 1: Shopping Behavior}
 \begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{fig/shopping_eval.jpg}
  \caption{Shopping evaluation caption}
  \Description{}
  \label{fig:shopping_eval}
\end{figure}

In the shopping behavior scenario, the experiment is designed to observe a subject during grocery shopping. We defined the grocery item list capturing the following categories: produce, liquids, animal products, frozen food, packaged food, seasoning, sauces, and junk food. The shopping list was designed to represent a variety of items from a western diet. The subject can interact with the item in 4 ways: taking the item into possession, putting the item back, inspecting the item, and standing in-front of the item without touching it. 
\medskip

\textbf{Data Collection:} The interface randomly assigns the item, method of interaction, pose, and the number of items to get between 1 to 5. The data collector informs the subject of the next assignment, tags the start of the activity, announces to the subject to start, and tags the end of the activity when the subject completes the assignment. To minimize mislabeling, the subject is first instructed to get close to the item to be interacted with before the label is tagged. To diversify the duration of interaction, subjects were in addition cued to either interact with the item quickly (<1 second) or for a longer duration (inspect the item for a self-determined 2-5 seconds). Each of the 3 visited one grocery store, with one of the participants visiting two grocery stores, providing data for 4 different grocery stores. In total, we collected 64 minutes and 57 seconds of data including 81837 frames. 

We observed 50 videos, where the participants adds items into his or her possession. 40 instances where he or she removed items from the possession and 40 instances of physical interaction and 38 instances for visual interaction with items. In total, participants interacted with 46 produce items, 20 packaged food items, 21 seasoning or sauce items, 28 animal products, 13 frozen food items, 27 junk food items and 29 liquids. 

%\medskip

%\textbf{Data Labeling:} We asked the labeler four questions. First is what is the INTERACTION. The kinds of interaction in the dataset includes inspecting an item visually without touching it (visual), physically inspecting an item (physical), taking the item into possession (add), and removing the item from possession (remove). Next, we ask the labeler what is the CATEGORY of the item. Category refers to the broader class that an item falls under. The full list of categories are listed in Figure \ref{fig:tree}. Based on the category selected, the labeler is then asked to choose the specific ITEM under the category. For example, under the category produce, the labeler is shown apples, bananas, peaches, strawberries, blueberries, lettuce, potatoes, onions, bell peppers, and broccoli. The list of items comes from the full list of items that were collected in our dataset as identified by the oracle. Finally, if the INTERACTION chosen is taking an item into possession, the labeler is also asked to count the number of items. 

\medskip

\textbf{Analysis:} We performed four analysis on the labeling performance: Category Level Classification, Item Level Classification, Interaction Classification, and In-hand Item Counting. 

\smallskip

 \noindent\underline{Categorical classification}. The human labelers had an average accuracy of 71\% for correctly labeling across 7 categories. For purposes of labeling performance, the precision metric is particularly crucial since we want to be able to trust that the labels are indeed what they say they are. When looking at the precision, we see that the average precision is 86\%, with 5 classes having >90\% precision. Packaged food is the only class that performed lower than 80\%, with a fairly low 47\%. This may be a case where the semantic of packaged food is unclear since technically most of the food items were indeed "in a package" so could have been misconstrued as "packaged food." In contrast, the recall is comparatively low, with an average of 70\%, and only 2 classes having >90\% recall. A low recall may not be as big of an issue given that we included a None of the Above case, with most of the missed instances falling under the None class. That means that some categories people are less confident about, for example liquids and junk food are largely missed as None. 

\begin{figure}[ht!]
  \centering
  \includegraphics[width=\linewidth]{fig/shopping_analysis.jpeg}
  \caption{We evaluate the shopping scenario with four different analysis. We evaluate the body motion that is happening (a), the item count (b) and the product category for the chosen item (c). We also evaluate the actual item, which can be seen in the appendix.}
  \Description{}
  \label{fig:shopping_analysis}
\end{figure}

\smallskip

 \noindent\underline{Item classification}. When asked to identify within the category what the actual item, the average labeling accuracy drops to 59\% across 41 classes. This decrease in accuracy seems mostly attributed to a reduction in recall through labeling items as None of the Above rather than inter-class mislabeling. The average recall dropped to \TODO[value], with \TODO[percent of incorrect] attributed to labeling as None. In comparison, the precision actually increased to an average of \TODO[value], with X number of classes above 90\%. 

One surprising observation we made is that certain items like spices were correctly labeled at a high rate, but when the investigators watched the videos ourselves, it was actually pretty difficult to tell what was in the person's hand. We believe that labelers were able to intuit what is in a person's hand based on the surrounding items in the shelf. Some of these items are particularly small, such as a box of black pepper. But the shelf has many units with the black pepper having a distinctive red top, white box in the American market. 

\smallskip

\noindent\underline{Shopper interaction}. We observe an accuracy of 91\% across four possible interactions: adding an item into a person's possession, removing the item into a person's possession, inspecting the item physically, and inspecting the item visually. Again None of the Above is a possible label. We can see that there is some confusion between visual inspection and that labelers chose to not classify the given instance as a visual inspection. This is likely because visual inspection in the PAR view looks as if the person is just standing in-front of the item. Without actually tracking the eyes of the subject, such an interaction cannot be differentiated from just standing in-front of the item. 

\smallskip

 \noindent\underline{Item counting}. Subjects were instructed to grab from 1 to 5 of the same item. The number of items a user held in their hand was counted correctly with an accuracy of 94\%, with a pearson correlation coefficient of $R = 0.93$ and $RMSE = 0.56$ (Figure \ref{fig:corrob}). We can see that labelers tend to under predict the amount of items chosen by the user. This might be due to the fact that items could be hidden below other items. Figure \ref{fig:ex_miscl} shows an instance of the user holding two pizzas, however only one is visible because they are stacked. 

%=========================Scenario 2 ===========================%
\subsection{Scenario 2: Exercise Tracking}
 \begin{figure}[ht!]
  \centering
  \includegraphics[width=\linewidth]{fig/exercise_eval.jpg}
  \caption{eating evaluation caption}
  \Description{}
  \label{fig:exercise_eval}
\end{figure}

In the exercise activity scenario, the experiment is designed to observe a subject doing a variety of exercises in an indoor gym environment. We are interested in seeing how well PAR captures the exercise being performed both in terms of the different equipment and also body movement. We included typical movements trackable by accelerometer based systems, which typically includes hand movement or full body motion, such as arm curls, jumping jacks, treadmills. We also included more stationary movements that accelerometers don't typically perform well with, such as pushups, leg lifts, and biking. 

\medskip


\textbf{Data Collection:} We selected activities under four different categories of equipment: body weight, free weights, weight machines, and cardio machines. Under each equipment, a variety of different exercises were performed. Activities that are repetition based (e.g. push-ups, bicep curls) are performed for ten repetitions. Activities on cardio machines are performed for one minute. Exercises were performed in a randomized sequence. The exercise assignment is announced to the subject in the same way as the shopping activity.

In total, we collected data from 6 people in 4 different gyms. For all repetition based exercises, the participants performed 498 repetitions in total. The whole data set is 49 minutes and 13 seconds long and contains 62013 frames.

%\medskip


%\textbf{Data Labeling:} We asked the labeler three questions. First is what is the exercise EQUIPMENT being used, which includes body weight, free weights, weight machines, and cardio machines. Next, based on the equipment chosen, a more detailed EXERCISE list is presented. For example, if the labeler chose body weight, the list presented includes plank, leg lift, jumping jacks, pull ups, push ups, mountain climber, and sit ups. Finally, if the exercise chosen is one that has REPETITIONS, such as push ups or bicep curls, the labeler is asked to count the number of repetitions. 

\medskip


\textbf{Analysis:} We performed three analysis on the labeling performance: Exercise Equipment Classification, Exercise Move Classification, and Repetition Counting. 

 \begin{figure}[b]
  \centering
  \includegraphics[width=\linewidth]{fig/exercise_analysis.jpeg}
  \caption{We evaluate the exercise scenario with three different concepts. First, we label the equipment (a), then we label the movement (c) and the number of repetitions (b) that the user performed.}
  \Description{}
  \label{fig:exercise_analysis}
\end{figure}

\smallskip

 \noindent\underline{Equipment classification}. When asked to identify the exercise based on the equipment used, the labelers accurately labeled exercise by the equipment used 85\% of the time. Again, just like the shopping analysis, precision in this case stands as the more crucial metric. The average precision is 94\%, with only one class (weights machine) lower than 95\% precision. For the most part, most of the confusion came down to labeling as None of the Above, leading to a comparatively low recall of 85\%. 

\smallskip

\noindent\underline{Exercise Move Classification}. When asked to identify within the equipment chosen what the actual exercise move is, the average labeling accuracy drops to 70\% across the the 17 exercise moves. Similar to the shopping item classification, this decrease in accuracy seems mostly attributed to a reduction in recall through labeling items as None of the Above rather than inter-class mislabeling. The average recall dropped to \TODO[value], with \TODO[percent of incorrect] attributed to labeling as None. In comparison, the precision stayed high at 91\%, with 12 out of 17 classes above 90\%. 

Looking closer at the confusions, some of the lowest recall activities included pull ups (44\%), mountain climbers (11\%), and leg lifts (30\%) were all body weight exercises. When the investigation team watched the videos ourselves, we also recognize that these videos are particularly difficult to interpret. The pull-ups were mostly mislabeled as an arm machine. This likely occurred with the way our labeling occurs in an hierarchical way where the labeler first chooses the equipment and then the specific exercise move. For mountain climbers and leg lifts, the actual activity is happening at the leg. For mountain climbers, the leg movement is only seen if the person is looking straight down or back down at the leg. Leg lifts, as seen in Figure\ref{fig:exercise_eval}, shows a somewhat difficult to interpret scene where the leg moves to and away from the body, which mostly got labeled as None of the Above. It is possible because labelers were not shown any examples of what an exercise looks like in tha PAR view, some of these less obvious body movements are not understandable. 

What is particularly promising about this result is that the performance remained relatively high for the wide variety of exercise types that was tested. As seen in the variety of classes, subjects performed exercises that have repetitions, but also exercises that are stationary like the body plank. Many exercises where an accelerometer based system would struggle, such as push-ups and biking, the PAR view captures them clearly. We imagine that a sensor fusion approach with motion measurements augmented with the PAR view for scene clarification would be able to capture all exercise movements near perfectly. 

\smallskip


 \noindent\underline{Reptition counting}. Subjects were instructed to perform exercises that are repetition based for 10 repetitions. Labelers, when shown a partial segment of the 10 exercises containing a random number of repetitions, counted the number of repetitions correctly with an accuracy of 89\%, with a pearson correlation coefficient of $R = 0.81$ and $RMSE = 1.83$ (Figure \ref{fig:corrob}). 85\% of the total incorrect rep count instances were +/- 1 rep from the true count. Initially, we had anticipated counting results to be much closer to perfect given how visually obvious the repetitions of an exercise can be seen in our initial pilot study. Upon closer reviewing of exercise videos, we noted that when subjects naturally exercised, the wearer often turned their head in the middle of the exercise. This leads to a change of what part of the body is in the frame. For arm-based exercises, it means that sometimes the arm goes in and out of the frame, which likely led to miscounting. 
 
%=========================Scenario 3 ===========================%
\subsection{Scenario 3: Dietary Monitoring}
 \begin{figure}[b]
  \centering
  \includegraphics[width=\linewidth]{fig/eating_eval.jpg}
  \caption{eating evaluation caption}
  \Description{}
  \label{fig:eating_eval}
\end{figure}

\smallskip


\textbf{Data Collection:} In the eating activity scenario, the experiment is designed to observe a subject during a eating situation where they freely consume food item of their choice (i.e. ordered food, self-prepared food, or snack). We observed each person within a 5-minute eating interval and annotate each bite and sip. o add additional complexity to the data, we also collected instances of the subjects just bringing their hand to their face without eating or drinking. The general content for food items were annotated, along with the time-stamp of each time the hand comes to the mouth. We additionally labeled the user's context while eating, focused on if the person is seated, standing, walking, or commuting in-vehicle while eating. 

One of the eating session was conducted in a shared dining environment of 8 people sitting around the table. This session is used to to observe how well the PAR view can capture company of others during meals.

We captured data from one barbeque session, where the participants consumed grilled meat and vegetables, bread and different salads. We additionally captured data from two restaurant sessions, where the participants consumed food items such as a sandwich, tacos, burgers, french fries and salads and drank soda and water. We captured six snacking sessions with items such as salty snacks, cookies, nuts, fruit (tangerines, apples, strawberries and bananas) and vegetables (snack tomatoes and carrots). We also observed two participants eating their self prepared food, such as salads, oatmeal, sandwiches or a curry and drinking coffee or wine. 

In total, we observed 24 different food items and 5 different drink items. We observed 148 bites, 35 sips and 20 touch face events. In total, we collected 64 minutes and 57 seconds of data including 81837 frames in 14 different locations. 

\smallskip


%\textbf{Data Labeling:} All eating moments were observed on a one to one basis with the experiment designer. All eating moments were labeled before the participant started eating by tagging the if the food contained fruit, meat or vegetables or if it was a salty snack, sweets of any kind or a fast food item. The experiment designer also annotated the food name for future reference. When the participant started eating, the experiment designer labeled each bite sip or touch face by annotating a specific timestamp in the video with the respective label. This enables a subsequent event extraction for every single bite or sip and also enables to track the amount of bites and sips the participant performed. To determine the presence of company, the experiment designer post labeled every frame in the video where a body part of one of the surrounding people was present in the video for more than 5 subsequent frames. 
%\smallskip

\textbf{Analysis:} We performed three analysis on the crowd labeling performance: eating motion classification, food content identification, and context of eating. Finally we analyze the percentage of time the PAR view captures people sitting around a table during meal.
\smallskip

\noindent\underline{Eating Motion Classification}. When asked to identify the hand to face motion, the labelers accurately distinguished between taking a bite, having a sip, and just touching the face with 94\% accuracy. All classes achieved above 96\% precision. Face touching is the most misconstrued class with the lowest recall of 81\% and 96\% precision.  

\begin{figure}[h!]
  \centering
  \includegraphics[width=\linewidth]{fig/eating_evaluation.jpeg}
  \caption{eating evaluation caption}
  \Description{}
  \label{fig:eating_analysis}
\end{figure}

\smallskip

\noindent\underline{Food Content Identification}. For the eating motion instances where the labeler identified as sips or bites, they are then asked to identify if a certain food content is in the scene. Because each food instance may contain more than one food content, they can select more than one category. As seen in Figure \ref{fig:eating_eval}, the average precision is much higher than average recall, 85\% compared to 62\%. For examples of salty snacks and sweets, most of our examples are food items that are quite small (e.g. nuts, gold fish crackers). Even the research team when reviewing the videos are only able to confidently identify what was being eaten by looking at the package or plate and not what was in the hand at the time of consumption. We speculate that this was likely the case for the crowd labelers given the fairly high precision score. This is an interesting advantage of the PAR view as compared to a more face focused visual view. PAR is able to provide simultaneously when food is being placed in the mouth, but also provide the scene of the table which often contains the plate or packaging, giving more context that can be used to disambiguate. We discuss this in more detail in the discussion section. 

\smallskip

\noindent\underline{Eating Context Classification}. For eating context, we focused on the context of eating in terms of if they are seated, standing, walking, or in a vehicle while as a passenger or driver eating. These contexts were classified correctly by the labelers with an accuracy of 88\%. We can see some confusion between walking and standing.


\smallskip

 \noindent\underline{Presence of Company}. For examining the ability of the PAR view at capturing the presence of company, we looked at how often a person would be in view if they were seated at different locations when the wearer is eating. The camera is on the right corner of the glasses, so the left side view is more obstructed. Figure \ref{fig:eating_context}b shows the position of the different people. The person to the right is most frequently in the frame, with 95\% of the total 5 minute of the eating session where the oracle identified the person is identifiable. The person to the left is least frequently in the frame at 11\%. The person to the front is captured at 5\%. The person to the left and to the front appear in the frame when the wearer moves their head between bites or redirects their attention, say during conversation. Hands can also show up in the frame. The table we chose is about 2 meters in diameter. For a smaller dining table, we imagine the person sitting across would be in the frame more frequently. However, because the purpose of knowing if there is company during eating is not to track the behavior of others but rather just to determine the presence of others, even at the lowest frequency of identification of the opposite side of the camera (in this case the left side), even in a 5 minute eating session, the person is seen at least a few times. 
 
 
 \begin{figure}[h!]
  \centering
  \includegraphics[width=\linewidth]{fig/eating_context.jpeg}
  \caption{(a) Confusion matrix for the eating context classification. (b) Percentage of body parts visible in frames captured by the PAR view for people sitting next to and across the participant. }
  \Description{}
  \label{fig:eating_context}
\end{figure}

\subsection{Scenario Differentiation}
Finally, we performed an analysis of how visually differentiable are the scenarios. For each of the scenarios, the crowd-sourced labelers are asked to identify which scenario (shopping, exercise, eating) best describes the video. By being able to automatically determine the scene, we can imagine using the PAR view to automatically determine which virtual sensor may be the best one to use. The labeler's reached near perfect scene differentiation, with an accuracy of 98\%. Precision was 100\%, with only a single cross-class missed classification. The drop in accuracy was only observed where labeler's labeled an instance as None of the Above, which lowered the recall to 97\%. Intuitively, this results is quite expected since our three scenarios are quite different and the task for differentiation is likley pretty easy. Visually the grocery store is quite different from the gym and eating instances always have food related items present. Nevertheless, the results are promising that human labelers that have never seen the PAR view can likely identify what is going on in the scene. 


\begin{figure}[b]
  \centering
  \includegraphics[width=0.7\linewidth]{fig/scen_prf.png}
  \caption{Confusion matrix and precision, recall, f1-scores for experiments for contextual situation analysis. White boxes indicate zero values.}
  \Description{}
  \label{fig:scen_conf}
\end{figure}

==> _9.Conclusion.tex <==
\section{Conclusion}

This paper evaluates the suitability of a Personal Action Radius Sensor for contextual analysis. Our work explains the use of a downwards facing camera to represent a person's activity radius within an arm's length. We performed a grocery shopping, exercise and food experiment which captures a labeled and unlabeled data set including 87 minutes of labeled data showing grocery shopping, exercise and food intake scenarios. For the purpose of evaluation, we performed contextual classification using a human intelligence algorithm for situational, activities and their categorizations, pose, items and their categorizations and repetition recognition as well as on nutritional intake and food content evaluation. This setup enabled us to draw contextual connections between classes. 
We evaluated all experimental setups in detail to determine the boundaries of interpret-ability of our provided data. In summary we can say that human intelligence evaluation is bounded by regularities of occlusion and information gaps. However, most tasks were answered precisely by human intelligence workers. This means that if the task was classified using the given label suggestions by the experimental setup, we can be almost sure that the labeling is true. We however observe a lower recall for some evaluations. This implicates that a subsequent revision by the experiment designer is necessary for unclassified examples, which were indicated by a 'none' label from the human intelligence worker in our study. We can also see that an experiment setup with smaller class clusters yields better results than bigger setups. Figure \ref{fig:overview_acc} shows an overview of all performed exercises and its accuracies. Using our proposed human intelligence algorithm, we saw that an almost perfect classification accuracy dropped with a finer granularity of the task. We were however able to conclude that human classification is able to correctly classify, and thus label the conceptual data proposed in this paper. 
